On Task-personalized Multimodal Few-shot Learning for Visually-rich Document Entity Retrieval

Visually-rich document entity retrieval (VDER), which extracts key information (e.g. date, address) from document images like invoices and receipts, has become an important topic in industrial NLP applications. The emergence of new document types at a constant pace, each with its unique entity types, presents a unique challenge: many documents contain unseen entity types that occur only a couple of times. Addressing this challenge requires models to have the ability of learning entities in a few-shot manner. However, prior works for Few-shot VDER mainly address the problem at the document level with a predefined global entity space, which doesn't account for the entity-level few-shot scenario: target entity types are locally personalized by each task and entity occurrences vary significantly among documents. To address this unexplored scenario, this paper studies a novel entity-level few-shot VDER task. The challenges lie in the uniqueness of the label space for each task and the increased complexity of out-of-distribution (OOD) contents. To tackle this novel task, we present a task-aware meta-learning based framework, with a central focus on achieving effective task personalization that distinguishes between in-task and out-of-task distribution. Specifically, we adopt a hierarchical decoder (HC) and employ contrastive learning (ContrastProtoNet) to achieve this goal. Furthermore, we introduce a new dataset, FewVEX, to boost future research in the field of entity-level few-shot VDER. Experimental results demonstrate our approaches significantly improve the robustness of popular meta-learning baselines.

==> dataset.tex <==

% \section{Dataset} \label{appendix-dataset}



% Since there is no dataset specifically designed for the FVDER task defined in Section \ref{formulation}, we construct a new dataset, FewVEX, to benchmark and evaluate the meta-learning based FVDER. 

% \subsection{Collection of Entity Types and Documents} 

% First, we collect the entity types $\C$ associated with the task distribution $P(\T)$ and a set of document images $\D$ annotated by these entity types.
% % Currently, we use the existing data corpus, designed for tasks like key information retrieval or parsing, in which the location information of entities is available. There are two datasets that is widely used in document understanding. 

% We consider two source datasets that are widely used in normal large-scale document understanding tasks such as entity recognition, parsing, and information extraction. The first one is the Form Understanding in Noisy Scanned Documents (FUNDS) dataset \cite{jaume2019funsd} comprises 199 real, fully annotated, scanned forms, with a total of three types of entities (i.e., questions, answers, heads). The second one is the Consolidated Receipt Dataset for post-OCR parsing (CORD) dataset \cite{park2019cord}. CORD consists of 1000 receipt images of texts and contains 6 superclasses (menåu, void menu, subtotal, void total, total, and etc) which are divided into 30 fine-grained subclasses. For different entity types, the total numbers of entity occurrences over the CORD images are highly imbalanced, ranging from 1 occurrence of entity \texttt{``void menu (nm)''} to 997 occurrences of \texttt{``menu (price)"}. 

% From the two datasets, we obtain a combined source dataset denoted as $ \D$,
% % \begin{equation}
% %     \D=\{(X_{orig,j}, Y_{orig,j})\}_{j=1}^M,
% % \end{equation}
% which contains $1199$ unique document images with original annotations on 33 classes.
% However, we observe that some fine-grained classes in CORD occurs in less than $max_i(M_{si}+M_{qi})$ images, the maximum number of documents within individual tasks. This will result in a large amount of repetitive usage of the same documents within one task and between different tasks. Therefore, we further sort the 33 classes by the number of unique document images where they occur and then discard three entity types that occurs in low frequency. 

% To sum up, we finally have a total of $|\C|=$30 entity types and $|\D|=1199$ unique document images annotated by these entity types. The pie chart (on the left) in Figure \ref{fig:dataset} illustrates the number of occurrences of the final entity types.



% % \begin{table*}
% % \small
% % \centering
% % \begin{tabular}{lcccccc}
% % \hline
% % \textbf{Benchmark Settings} & \textbf{Train Source} & \textbf{Test Source} & \textbf{$|\C_{base}|$ }& \textbf{$|\C_{novel}|$} &\textbf{\#Train Tasks}  &\textbf{\#Test Tasks}  \\
% % \hline
% % % \text{FVDER (ITD)} & - & CORD & 0 & 31 & 0 & 3000 \\
% % \text{FVDER (CROSS)}  & CORD  & FUNSD & 27 & 3 & 3600 & 300 \\
% % \text{FewVEX(M)}  &  CORD+FUNSD &  CORD+FUNSD & 24 & 7 & 3000 & 800 \\
% % \hline
% % \end{tabular}
% % \caption{Statistics of the three benchmark settings based on the FVDER dataset.}
% % \label{tab:dataset}
% % \end{table*} 


% \subsection{Collection of Training and Testing Tasks} 
% Second, we create a meta-learning dataset $\D_{meta}=\{\D_{meta}^{trn}, \D_{meta}^{tst}\}$, consisting of a meta-training set $\D_{meta}^{trn}$ containing $\tau_{trn}$ training tasks and a meta-testing set $\D_{meta}^{tst}$ containing $\tau_{tst}$ testing tasks. Each task instance follows the N-way K-shot FVDER task setting. An overview of dataset construction is in Figure \ref{fig:dataset}.
% % and can be also called an \textit{episode} as in \cite{chen2021meta}. 




% \subsubsection{Entity Type Split} 
% To ensure that testing tasks in $\D_{meta}^{tst}$ focus on novel classes that are unseen during meta-training $\D_{meta}^{trn}$, we should split the total entity types $\C$ into two separate sets $\C =  C_{base} \cup \C_{novel}, \C_{base} \cap \C_{novel} = \emptyset$ such that
% $\C_{base}$ is used for meta-training and $\C_{novel}$ for meta-testing.
% % $\D_{meta}^{trn}$ and $\D_{meta}^{tst}$. focus on two separate sets of entity types. 

% Specifically, we use a split ratio $\gamma$ to control the number of novel classes and randomly choose $\gamma|C|$ entity types from $\C$ as $\C_{novel}$. Then, $\C_{base} = \C \setminus \C_{novel}$. 
% % Note that for parallel computing, different processes share the same split C = {Cbase, Cbase}. 
% % Then, we can use the class pool (a list of entity type IDs), Cbase  or Cnovel, to point to a combination of related candidate datasets. 
% Note that for the cases that some entity types occurs in less number of documents than the others, we set a threshold $U$ and any entity type that occurs in less than $U$ documents are forced to be one of the novel classes. 
% % In this paper, we set $\gamma=0.4$ and $U=10$.
% % by removing them in the
% % For fair split of classes, w
% % sort the entities by document number where they occur
% % remove the entities with less than 2K documents.






% \subsubsection{Single N-way K-shot Task Generation} \label{dataset:task-gen}



% Each individual task $\T=\{S, Q, \E \}$ in either $\D_{meta}^{trn}$ or $\D_{meta}^{tst}$ can be generated by the following steps (summarized in Algorithm \ref{alg:algorithm}).

% \paragraph{Class sampling.} The target classes of task $\E$ is generated by randomly sampling $N$ entity types from either $\C_{base}$ (for the training task) or $\C_{novel}$ (for the testing task).



% \paragraph{Document sampling.} Given the $N$ target classes, we then collect document images that satisfies the few-shot setting defined in Section \ref{task-setting}. However, one problem of document sampling from the original corpus is the \textit{inefficiency}. It is because, for each task, only a small number of documents that contain the corresponding classes can be the candidate documents of the task. 
% For example, if each document contains only a small number of entity types,
% % (for example, a document has only 3 entity types but the class pool has 30 types),
% the majority of documents would be rejected.
% To improve sampling efficiency, one strategy is to count entities in each document in advance and, for each entity type, all the candidate documents that contain this type are temporally stored in a new dataset. Then, we only look at the task-specific candidate datasets $\D^{\E}= \{\D^e | \forall e \in \E\} $, where $\D^e = \{(X,Y)| \forall (X,Y) \in \D  \text{ if } e \in Y\}$.
% % $\D_{\E_i}=\{\D_e | \forall e \in \E_i\}$, where $\D_e = \{(X,Y)| \text{if }e \in Y, \forall (X,Y) \in \D \}$.  
% % , we can sample documents more efficiently. 
% Specifically, we randomly sample $M_{s}$ documents such that the total number of entity instances is satisfied--that is, $K \sim \rho K$ shots per entity type. Likewise, we sample $M_{q}$ documents for $Q$, such that there are $K_q \sim \rho K_q$ shots per entity type. We keep track a table to record the current count of occurrences of each type of entity types in the task. 
% % Note that $S_i \cap Q_i = \emptyset$.  

% \paragraph{Label Conversion.}
% In the few-shot setting, the majority region of an document does not follow the \textit{in-task distribution} (ITD) of $\E$. These regions' tokens are treated as either background or the other types of entities from the \textit{out-of-task distribution} (OTD), whose original labels should be arbitrarily converted into \texttt{O} label. In addition, we map the original labels of ITD tokens to relative labels. 
% For example, if we use I/O schema, the relative labels should range from label id 0 to label id $(N-1)$.
% % If we use B/I/O setting

% % 3) \textbf{Multimodal Input Features} Layout structure
% % graph of boxes, beta-skeleton
% % need a figure





% \begin{algorithm}[h]
% %   \vspace{-0.03in}
%     \small
%    \caption{Single FVDER Task Generation}
%   \begin{algorithmic}[1]
%     \STATE \textbf{Require:} $N, K, K_q, \rho$, $\C_{base}$, $\C_{novel}$, $\D$.
%     \STATE Randomly sample $N$ entity types from either $\C_{base}$ or $\C_{novel}$ and obtain $\E$.
%     \STATE \textbf{Initialize:} $S=\emptyset$, $Q=\emptyset$
%     \STATE \textbf{Initialize:} $\D^{\E}= \{\D^e | \forall e \in \E\} $ from $\D$.
%     % = \{(X,Y)| \forall (X,Y) \in \D  \text{ if } e \in Y\}$ for $\forall e \in \E$
%     \STATE \textbf{Initialize:} $N$ integers $train\_count[e]=0$ for $\forall e \in \E$.
%     \STATE \textbf{Initialize:} $N$ integers $test\_count[e]=0$ for $\forall e \in \E$.

%     \STATE // Document sampling for $S$
%     \WHILE{$\min_{e \in \E} train\_count[e] < K $}
%         \STATE Find the least frequent entity type in the current task, i.e., $\hat{e}= \text{argmin }_{e \in \E} train\_count[e] $.
%         \STATE Sample a document $(X_j, Y_j)$ from $\D^{\hat{e}}$
%         \STATE Add $(X_j, Y_j)$ to $S$
%         \FOR{$e \in \E$}
%             \STATE Remove the selected document from candidate dataset $\D^{e} \xleftarrow[]{} \D^{e} \setminus \{(X, Y)\}$
%             \STATE Update $train\_count[e]$ if $Y$ contains entity type $e$.
%             \IF{$train\_count[e] > \rho K$}
%                 \STATE Mask $(train\_count[e] - \rho K)$ instances of type-$e$ by setting token labels to -1
%             \ENDIF
%         \ENDFOR
%     \ENDWHILE

%     \STATE // Document sampling for $Q$
%     \WHILE{$\min_{e \in \E} test\_count[e] < K_q $}
%         \STATE Find the least frequent entity type in the current task, i.e., $\hat{e}= \text{argmin }_{e \in \E} test\_count[e] $.
%         \STATE Sample a document $(X_j, Y_j)$ from $\D^{\hat{e}}$
%         \STATE Add $(X_j, Y_j)$ to $Q$
%         \FOR{$e \in \E$}
%             \STATE Remove the selected document from candidate dataset $\D^{e} \xleftarrow[]{} \D^{e} \setminus \{(X, Y)\}$
%             \STATE Update $test\_count[e]$ if $Y$ contains entity type $e$.
%             \IF{$test\_count[e] > \rho K_q$}
%                 \STATE Mask $(test\_count[e] - \rho K_q)$ instances of type-$e$ by setting token labels to -1
%             \ENDIF
%         \ENDFOR
%     \ENDWHILE
%     \STATE Label conversion for $\forall (X_j, Y_j) \in S \cup Q$.
%     % \STATE  Add $\T_i=\{S_i, Q_i, \E_i\}$ to $\D_{meta}^{trn}$.
%     % \ENDFOR
%     % \FOR{$i=1,2,...,\tau_{tst}$}
%     %     \STATE Randomly sample $N$ entity types from $\C_{novel}$ as $\E^*_i$.
%     %     \WHILE{}
%     %     \ENDWHILE
%     %     \STATE Add $\T^*_i=\{S^*_i, Q^*_i, \E^*_i\}$ to $\D_{meta}^{test}$.
%     % \ENDFOR
%     \STATE \textbf{return:} $\T=\{S, Q, \E\}$
%   \end{algorithmic}
%   \label{alg:algorithm}
% \end{algorithm}


% \subsection{Dataset Variants} \label{dataset-benchmark}
% We fix the testing shot as $K_q$=4. We propose two variants of meta-dataset, each of which pay attention to different challenges in few-shot learning. The statistics is summarized in Table \ref{tab:benchmark}:
% \textbf{FewVEX(S)} focuses on single-domain receipt understanding under N-way K-shot setting. The training and testing classes are both from CORD. The goal is to learn domain-invariant meta-parameters.
% \textbf{FewVEX(M)} focuses on learning domain-agnostic meta-parameters from a combination of receipt and form understanding.
% % The training classes consists of 18 in CORD and 2 classes in FUNSD, while the testing classes contains the unseen 5 classes in CORD and 1 in FUNSD. 
% Receipt and form documents may appear in the same task.
% % (3) \text{FVDER (CROSS)} also aims to learn domain-agnostic meta-parameters, though focusing on the transferability of our model between different document domains (i.e., from receipts to forms). The training classes is limited to one domain but applied to a totally-unseen domain. 
% % % Training tasks are from receipt domain, while the testing tasks are from the form domain. Noting that since FUNSD only has three entity types (i.e., $|\C_{novel}|=3$), we can only conduct experiments with task setting $N<=3$.


% \begin{table*}
% \small
% \centering
% \begin{tabular}{lccccccc}
% \hline
% \multirow{2}{*}{\textbf{Datasets}} & \multicolumn{3}{c}{\textbf{Meta Training}} & \multicolumn{3}{c}{\textbf{Meta Testing}} & \textbf{Range}\\
% \cmidrule(lr){2-4}
% \cmidrule(lr){5-7}
%  & \textbf{Domains} & \textbf{\# Entity Types} &\textbf{\# Tasks}  & \textbf{Domains} & \textbf{\# Entity Types} & \textbf{\# Tasks}  & \textbf{of N} \\
% \hline
% % \text{FVDER (C)}  & CORD & 23 & 3600 & FUNSD & 3  & 64 \\
% \text{FewVEX(S)} & CORD & 18 & 3000 & CORD & 5  & 128  & [1, 5] \\
% \text{FewVEX(M)} & CORD+FUNSD  & 20 & 3000 &  CORD+FUNSD & 6 & 256  & [1, 6] \\
% \hline
% \end{tabular}
% \caption{Statistics of two FVDER datasets. Testing entity types are unseen in training tasks. From each dataset, we can test different $N$-way $K$-shot settings.}
% \label{tab:benchmark}
% \end{table*} 


